Gravitational collapse of plasmas in General Relativity

We provide a covariant derivation of plasma physics coupled to gravitation by utilizing the 3+1 formulation of general relativity, including a discussion of the Lorentz force law. We then reduce the system to the spherically symmetric case and show that all regions of the spacetime can be represented in a single coordinate system, thus revoking the need for junction conditions. We further show that the region exterior to the collapsing region is naturally described by the charged Vaidya spacetime in non-null coordinates.

==> new_commands.tex <==
\newcommand{\da}{\partial}
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\de}{\delta}
\newcommand{\De}{\Delta}
\newcommand{\ga}{\gamma}
\newcommand{\ep}{\varepsilon}
\newcommand{\si}{\sigma}
\newcommand{\Si}{\Sigma}
\newcommand{\la}{\lambda}
\newcommand{\La}{\Lambda}
\newcommand{\ka}{\kappa}
\newcommand{\curl}{\textrm{curl}}
\newcommand{\om}{\omega}
\newcommand{\sch}{Schwarzschild}
\newcommand{\Om}{\Omega}
\newcommand{\ks}{Kruskal-Szekeres }
\newcommand{\M}{\mathcal{M}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\U}{\mathcal{U}}
\newcommand{\V}{\mathcal{V}}
\newcommand{\Lie}{\mathcal{L}}
\newcommand{\nR}{{^{\sst{(n)}}R}}
\newcommand{\mR}{{^{\sst{(m)}}R}}
\newcommand{\nminoneR}{{^{\sst{(n-1)}}R}}
\newcommand{\nminoneQ}{{^{\sst{(n-1)}}Q}}
\newcommand{\nC}{{^{\sst{(n)}}C}}
\newcommand{\nminoneC}{{^{\sst{(n-1)}}C}}
\newcommand{\mE}{{^{\sst{(m)}}E}}
\newcommand{\mB}{{^{\sst{(m)}}B}}
\newcommand{\nQ}{{^{\sst{(n)}}Q}}
\newcommand{\EFE}{Einstein's Field Equations}
\newcommand{\nka}{{^{\sst{(n)}}\ka}}
\newcommand{\ts}{\textstyle}
\newcommand{\sst}{\scriptscriptstyle}
%\newcommand{\R}{\widetilde{R}}
\newcommand{\fourR}{{^{\sst{(4)}}R}}
\newcommand{\fourQ}{{^{\sst{(4)}}Q}}
%\newcommand{\C}{\widetilde{C}}
\newcommand{\fourC}{{^{\sst{(4)}}C}}
%\newcommand{\Q}{\widetilde{Q}}
%\newcommand{\K}{{\widetilde{K}}}
%\newcommand{\trK}{tr\widetilde{K}}
\newcommand{\Nabla}{\widetilde{\nabla}}
%\newcommand{\G}{\widetilde{G}}
\newcommand{\fiveka}{\widetilde{\ka}}
%\newcommand{\T}{\widetilde{T}}
\newcommand{\fiverho}{\widetilde{\rho}}
\newcommand{\fivePi}{\widetilde{\Pi}}
\newcommand{\fiveS}{\widetilde{S}}
%\newcommand{\A}{\widetilde{A}}
\newcommand{\fivej}{\widetilde{j}}
\newcommand{\fiveP}{\widetilde{P}}
%\newcommand{\E}{\widetilde{E}}
%\newcommand{\B}{\widetilde{B}}
\newcommand{\hs}{\hspace{0.15cm}}
\newcommand{\fiveR}{\widetilde{R}}
\newcommand{\threeR}{{^{\sst{(3)}}R}}
\newcommand{\threeQ}{{^{\sst{(3)}}Q}}
\newcommand{\fiveal}{\widetilde{\al}}
\newcommand{\fivebe}{\widetilde{\be}}
\newcommand{\Al}{\widetilde{\al}}
\newcommand{\Be}{\widetilde{\be}}
\newcommand{\detf}{det\, f}
\newcommand{\detg}{det\, g}
\newcommand{\deth}{det\, h}
\newcommand{\W}{\widetilde{W}}
\newcommand{\el}{\ell}
\newcommand{\Dp}{D$p$}
\newcommand{\SZ}{${\bf S}^1/{\bf Z_2}$}
\newcommand{\D}{\Lie_n}
\newcommand{\Real}{{\bf R}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\zetabar}{\bar{\zeta}}
\newcommand{\betabar}{\textrm{\b{$\beta$}}}
\newcommand{\eem}{EM}
\newcommand{\fluid}{F}
\newcommand{\Tem}{T^{\eem}}
\newcommand{\rhoem}{\rho^{\eem}}
\newcommand{\Pem}{P^{\eem}}
\newcommand{\jem}{j^{\eem}}
\newcommand{\Piem}{\Pi^{\eem}}
\newcommand{\Tmat}{T^{\fluid}}
\newcommand{\rhomat}{\rho^{\fluid}}
\newcommand{\Pmat}{P^{\fluid}}
\newcommand{\jmat}{j^{\fluid}}
\newcommand{\Pimat}{\Pi^{\fluid}}
\newcommand{\Epar}{\E_{\parallel}}
\newcommand{\Bpar}{\B_{\parallel}}
\newcommand{\Er}{\E_{r}}
\newcommand{\Etheta}{\E_{\theta}}
\newcommand{\Ephi}{\E_{\phi}}
\newcommand{\real}{\mathbb{R}}
\newcommand{\that}{\hat{t}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\s}{\mathcal{S}}
\newcommand{\J}{\mathcal{J}}
\newcommand{\PP}{\mathcal{P}}
\newcommand{\E}{\mathcal{E}}
\newcommand{\B}{\mathcal{B}}
\newcommand{\Br}{{\B_{r}}}
\newcommand{\Btheta}{{\B_{\theta}}}
\newcommand{\Bphi}{{\B_{\phi}}}
\newcommand{\Q}{\mathcal{Q}}
\newcommand{\rAH}{r_{\pm}}
\newcommand{\scri}{\mathscr{I}}
\newcommand{\what}{\hat{\hat{w}}}
\newcommand{\wbar}{\hat{w}}
\newcommand{\wsq}{\tilde{w}}
\newcommand{\wsqsq}{\tilde{\tilde{w}}}
\newcommand{\Phat}{\hat{\hat{P}}}
\newcommand{\Pbar}{\hat{P}}
\newcommand{\Psq}{\tilde{P}}
\newcommand{\Psqsq}{\tilde{\tilde{P}}}
\newcommand{\ahat}{\hat{\hat{a}}}
\newcommand{\abar}{\hat{a}}
\newcommand{\asq}{\tilde{a}}
\newcommand{\asqsq}{\tilde{\tilde{a}}}
\newcommand{\qhat}{\hat{\hat{q}}}
\newcommand{\qbar}{\hat{q}}
\newcommand{\qsq}{\tilde{q}}
\newcommand{\qsqsq}{\tilde{\tilde{q}}}
\newcommand{\lahat}{\hat{\hat{\lambda}}}
\newcommand{\labar}{\hat{\lambda}}
\newcommand{\lasq}{\tilde{\lambda}}
\newcommand{\lasqsq}{\tilde{\tilde{\lambda}}}
\newcommand{\Bhat}{\hat{\hat{B}}}
\newcommand{\Bbar}{\hat{B}}
\newcommand{\Bsq}{\tilde{B}}
\newcommand{\Bsqsq}{\tilde{\tilde{B}}}
\newcommand{\ephat}{\hat{\hat{\epsilon}}}
\newcommand{\epbar}{\hat{\epsilon}}
\newcommand{\epsq}{\tilde{\epsilon}}
\newcommand{\epsqsq}{\tilde{\tilde{\epsilon}}}
\newcommand{\Pihat}{\hat{\hat{\Pi}}}
\newcommand{\Pibar}{\hat{\Pi}}
\newcommand{\Pisq}{\tilde{\Pi}}
\newcommand{\Pisqsq}{\tilde{\tilde{\Pi}}}
\newcommand{\R}{\mathfrak{R}}

